AdVENTR: Autonomous Robot Navigation in Complex Outdoor Environments

We present a novel system, AdVENTR for autonomous robot navigation in unstructured outdoor environments that consist of uneven and vegetated terrains. Our approach is general and can enable both wheeled and legged robots to handle outdoor terrain complexity including unevenness, surface properties like poor traction, granularity, obstacle stiffness, etc. We use data from sensors including RGB cameras, 3D Lidar, IMU, robot odometry, and pose information with efficient learning-based perception and planning algorithms that can execute on edge computing hardware. Our system uses a scene-aware switching method to perceive the environment for navigation at any time instant and dynamically switches between multiple perception algorithms. We test our system in a variety of sloped, rocky, muddy, and densely vegetated terrains and demonstrate its performance on Husky and Spot robots.

==> proposed_method.tex <==
Cost maps from outdoor perception
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth,height=3cm]{figs/perception_costmaps.png}
    \caption{\small{Navigation cost maps generated from our perception modules. (a) An elevation cost map from TERP \cite{weerakoon2022terp} that highlights higher elevations in light and lower elevations in dark colors; (b) Surface cost map generated from TerraPN \cite{sathyamoorthy2022terrapn} for a given RGB input. High costs in light colors indicate rough/granular terrains that lead to vibrations. (c) Vegetation cost map generated from VERN \cite{sathyamoorthy2023vern} to identify pliable vegetation regions for a given RGB image quadrants(bottom left). Red quadrants indicate non-pliable/solid objects. }}
    \label{fig:perception_fig}
\end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Second Draft %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proposed Method}
In our framework, we treat autonomous outdoor robot navigation as a combined effort of robot perception and planning. Our perception module provides an understanding of the environmental challenges such as terrain elevation, surface condition (poor traction, granularity, etc), and pliability of the vegetation around the robot using raw sensory data. However, identifying such environmental conditions using a unified/single perception approach is non-trivial due to the complexity of the multi-modal data streams needed to be processed, the scale of the model (regardless of whether it is learning-based or model-based), and the associated computation requirements on-board the robot. Hence, we propose three separate perception sub-modules to identify terrain elevation, surface properties, and vegetation pliability respectively. The modules generate cost maps that quantify the navigability under each environmental condition. However, since the necessity of each perception sub-module varies from one environment to another, we propose a scene-aware switching mechanism to alternate between perception sub-modules to improve computational efficiency. Finally, we propose a planner that can generate navigation actions by incorporating the cost maps provided by our perception modules.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Second Draft %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% First Draft %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% In this section, we discuss the details of our method. We treat autonomous outdoor robot navigation as a combined effort of robot perception and planning. Our perception module provides an understanding of the environmental conditions such as terrain elevation, surface condition (poor traction, granularity, etc), and pliability of the vegetation around the robot using raw sensory data. However, identifying such environmental conditions using a unified perception approach is non-trivial due to the complexity of the data streams and sensors required to detect different conditions. Hence, we propose three separate perception sub-modules to identify terrain elevation, surface properties, and vegetation pliability respectively. The modules generate cost maps that quantify the navigability under each environmental condition.

% We observe that the necessity of each perception sub-module varies from one environment to another. For instance, terrain elevation perception is redundant in even/flat outdoor terrains where a robot can navigate without explicitly understanding terrain elevation. Hence, we propose a scene-aware switching mechanism between our perception sub-modules to improve computational efficiency by mitigating the use of redundant perception throughout the navigation. Finally, we propose a planner that can generate navigation actions by incorporating the cost maps provided by our perception modules. We summarize the technical details of our approach in the sub-sections below.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% First Draft %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Sensory Inputs}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Second Draft %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We utilize an RGB camera, a 3D LiDAR, Odometry, a 6-DOF IMU (for wheeled robots), and Joint feedback (for legged robots) sensors to perform scene understanding and navigability estimation during perception. We acquire the sensor data streams: RGB image ($I_t^{RGB}$), 3D point cloud ($P_t^{lidar}$), robot's position w.r.t the odometry frame ($x_t^O, y_t^O$), current linear and angular velocities ($v_t, \omega_t$), its orientation (i.e, roll ($\phi_t$), pitch ($\theta_t$), yaw ($\psi_t$) angles), IMU data vector ($V_t^{IMU}$), and leg joint feedback vector ($J_{t}$) for a legged robot at a given time $t$ to conduct several scene understanding and perception tasks summarized in the following sub-sections.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Second Draft %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Scene Understanding} \label{sec:scene-understand}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Second Draft %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Our framework's scene understanding module determines the predominant navigation challenge in the robot's immediate surroundings to utilize the appropriate perception method to handle it. To this end, we first analyze the robot's local sensing data and define three metrics $q_{uneven}, q_{rough}$ and $q_{pliable}$ to quantify the level of unevenness, roughness, and vegetation pliability of a terrain respectively.

\subsubsection{Terrain Unevenness:} We incorporate a robot-centric 2D elevation map $E_t \in [0,100]^{N \times N}$ generated from the 3D LiDAR point cloud $P_t^{lidar}$ using the ROS package in \red{cite Elevation mapping} to understand the unevenness of the terrain. We first calculate the gradient matrix $G_t^E$ of the elevation map $E_t$ to calculate the elevation gradients. Then, let $q_{uneven} \in [0,1]$ be the terrain unevenness factors calculated as $q_{uneven} = \big( max(G_t^E) - min(G_t^E) \big)/100$. 

\subsubsection{Terrain Surface Properties:} We quantify the terrain surface properties such as granularity and roughness using the factor $q_{rough} $. Since the wheeled and legged robots experience surface properties differently, we utilize IMU data and Joint data for wheeled and legged robots respectively to obtain $q_{rough}$. We observe that applying principal component analysis (PCA) \cite{sathyamoorthy2022terrapn} \cite{elnoor2023pronav} on the immediate history of IMU or Joint data enables us to understand the roughness of the surface. In particular, we observe that the variances of the first two principal components ($\sigma_{PC_1}, \sigma_{PC_2}$) after applying PCA on IMU or joint data quantifies the surface condition (See Fig. \ref{fig:scene_und_fig}.a). Hence, we calculate $q_{rough} = \sqrt{\sigma_{PC_1}^2+ \sigma_{PC_2}^2}$.
% Granularity - if the variance of PCA below a threshold, the terrain is smooth

\subsubsection{Terrain Vegetation Pliability:} Outdoor environments often include different types of vegetation. Some of these vegetation regions are pliable and safe to navigate due to lower density. We incorporate a 2D intensity map ($D_t \in [0,100]^{N \times N}$) generated from the 3D point cloud  $P_t^{lidar}$ to identify the existence of such pliable vegetation. Our intensity map $D_t$ represents the reflecting strength (i.e., intensity) of the LiDAR rays in the robot's vicinity. Higher intensities in $D_t$ indicate solid objects such as trees, bushes, etc while lower intensities represent less-dense objects such as thin vegetation. Hence, we calculate the vegetation pliability factor $q_{pliable} \in [0,1]$ as,  $q_{pliable}= \frac{N_p}{N_{tot}}$, where $N_p$ is the no. of grids in $D_t$ in the rage of 40-70 (i.e., intensity range for less-dense objects), and $N_{tot}$ is the total no. of grid points in $D_t$.
Vegetation - if the intensity map includes intermediate cost values, pliable vegetation might exist

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth,height=3cm]{figs/scene_understanding_fig.png}
    \caption{\small{Sensor data analysis for scene understanding and perception. (a) PCA analysis on IMU data (for wheeled robots) and Proprioception data (for legged robots). Granular terrains such as rocks (brown) and sand (orange) lead to high variances in the first two principal components (i.e., $\sigma_{PC_1}, \sigma_{PC_2}$). (b) LiDAR point cloud intensity map used to identify the existence of soft/pliable objects.}}
    \label{fig:scene_und_fig}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth,height=3cm]{figs/perception_costmaps.png}
    \caption{\small{Navigation cost maps generated from our perception modules. (a) An elevation cost map from TERP \cite{weerakoon2022terp} that highlights higher elevations in light and lower elevations in dark colors; (b) Surface cost map generated from TerraPN \cite{sathyamoorthy2022terrapn} for a given RGB input. High costs in light colors indicate rough/granular terrains that lead to vibrations. (c) Vegetation cost map generated from VERN \cite{sathyamoorthy2023vern} to identify pliable vegetation regions for a given RGB image quadrants(bottom left). Red quadrants indicate non-pliable/solid objects. }}
    \label{fig:perception_fig}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Second Draft %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% First Draft %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% A given outdoor environment can consist of one or more terrain conditions such as unevenness, granularity, and vegetation. Hence, it is important for an autonomous navigation algorithm to identify such different terrain conditions around the robot (i.e., scene understanding) to perform efficient perception and planning. To this end, we first analyze the robot's local sensing data to estimate the terrain conditions of the robot's vicinity summarized below. Here, we define three metrics $q_{uneven}, q_{rough}$ and $q_{pliable}$ to quantify the level of unevenness, roughness, and vegetation pliability of a terrain respectively.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% First Draft %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Outdoor Perception} \label{sec:perception}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Second Draft %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We provide an overview of the outdoor perception methods used in our framework in Table \ref{tab:perception}. TERP and VERN are robot agnostic, whereas TerraPN and ProNav are designed specifically for wheeled and legged robots respectively.

\begin{table}[h]
\centering
\begin{tabularx}{\linewidth}{|c|c|L|} % Change the alignment to center
\hline
\textbf{Method} & \textbf{Inputs} & \textbf{Outputs}  \\

\hline
TERP \cite{weerakoon2022terp} & $P_t^{lidar}$, $x_t^O, y_t^O$, $\phi_t, \theta_t, \psi_t$, $V_t^{IMU}$ & Cost map containing reduced-stability regions, risk of flip-over, etc. \\
\hline

TerraPN \cite{sathyamoorthy2022terrapn} & $I_t^{RGB}$, $v_t, \omega_t$ & Surface cost map for a wheeled robot encoding terrain's traction, bumpiness, granularity. \\ 
\hline

ProNav \cite{elnoor2023pronav} & $J_{t}$ & Surface cost map for a legged robot encoding terrain's traction, bumpiness, granularity. \\
\hline

VERN \cite{sathyamoorthy2023vern} & $I_t^{RGB}$ & Vegetation cost map classifying vegetation as tall grass, bushes, and trees.\\
\hline

\end{tabularx}
\caption{\small{Descriptions of the outdoor perception methods.}}
\label{tab:perception}
\vspace{-15pt}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Second Draft %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% First Draft %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% In this section, we discuss our methods for outdoor perception. The methods output cost maps that our planner integrates to compute \textit{optimal} velocities to alleviate challenges and reach the robot's goal. 

% \subsubsection{Terrain Elevation Perception: }
% % terp
% Our first objective is to tackle the geometric properties of outdoor terrains, i.e., their slope, unevenness, etc. To this end, we use TERP \cite{weerakoon2022terp}, a method that uses lidar point clouds, the robot's pose, and goal to compute an elevation-aware cost map of the environment. TERP trains an end-to-end DRL model that uses an elevation map E (obtained by processing point clouds) to compute an attention mask A that can be applied over the input elevation map E. The resulting masked cost map $(E x A)$ identifies and highlights the reduced-stability regions where the robot could have unstable poses (pitch and roll angles) or even topple.

% \subsubsection{Terrain Surface Condition Perception}
% Another challenge to outdoor navigation arises from a terrain's surface properties such as traction, bumpiness, granularity, etc that cause undesirable effects such as high vibrations, wheel/leg slip, entrapment in granular surfaces such as sand, mud, etc. To address this, we propose two methods: 1. TerraPN for wheeled robots, and 2. ProNav for legged robots. TerraPN \cite{sathyamoorthy2022terrapn} learns the surface properties (traction, bumpiness, deformability, etc.) of complex outdoor terrains directly from robot-terrain interactions through self-supervised learning. It uses RGB images of terrain surfaces and the robot's velocities as inputs, and the IMU vibrations and wheel odometry errors experienced by the robot as labels for self-supervision. TerraPN outputs a \textit{surface} cost map relative to the RGB image that differentiates smooth, high-traction surfaces (low navigation costs) from bumpy, slippery, granular surfaces (high navigation costs). 

% % ProNav
% Since wheeled and legged robots experience terrains differently, a new approach tailor made for legged robots is required. ProNav \cite{elnoor2023pronav} uses proprioception signals (data denoting the robot's body movements) to characterize terrain surfaces. It uses a legged robot's joint positions, forces, and current consumed by actuators to evaluate a terrain’s stability, resistance to its motion, risk of entrapment, and crashing. ProNav interfaces easily with any planner that uses exteroception (RGB images, lidar, etc) and outputs an appropriate stable gait for the robot to execute when the terrain becomes unstable.


% \subsubsection{Vegetation Pliability Perception}
% %vern, graspe
% % Another major challenge in outdoor navigation is differentiating pliable/traversable obstacles (e.g. tall grass) from non-pliable/hard obstacles (e.g. trees, buildings, etc). This would allow the robot to navigate densely vegetated and forested environments. To this end, we use VERN, a  

% To handle dense vegetation, differentiate pliable/traversable objects (such as tall grass) and non-pliable/hard obstacles such as trees, we use VERN \cite{sathyamoorthy2023vern}. VERN trains a classifier on quadrants divided from RGB images to classify vegetation in the scene as tall grass, bushes, or trees. The classification result along with its confidence, and vegetation height (extracted from lidar point clouds) are used to calculate a vegetation-aware cost map (\red{point to fig}).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% First Draft %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% First/Second Draft %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Planner}
Our framework uses a novel, generalized planner capable of interfacing with the perception methods described in section \ref{sec:perception}. We extend the Dynamic Window Approach (DWA) \cite{fox1997dynamic} to account for the elevation, surface, and vegetation costs while computing collision-free, goal-reaching, optimal linear and angular velocities $(v^*, \omega^*)$. To achieve this, we formulate a novel objective function (equation \ref{eqn:objective-func}) to find optimal velocities from the set of feasible robot velocities that are \textit{reachable} based on the robot's current velocities, and acceleration limits.  

\begin{gather}
    G(v, \omega) =  \alpha.\text{Head}.(1 - \textbf{Surface}) + \beta.\text{Obs} + \gamma.\text{Vel} + \delta.\textbf{Elevation} + \theta.\textbf{Veg}
    \label{eqn:objective-func}
\end{gather}

\no Here, Head() measures the progress towards the robot's goal, Obs() is the distance to the closest obstacle when executing a certain $(v, \omega)$,  Vel() measures the forward velocity of the robot and encourages higher velocities, Surface() denotes the surface cost from obtained from TerraPN, Elevation() represents the elevation cost from TERP, and Veg() is the vegetation cost from VERN. The highlighted terms are added newly as part of our formulation. They are used depending on our scene understanding module which activates a perception module based on the detected navigation challenge in the environment. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% First/Second Draft %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
